Paternalism, Autonomy, or Both? Experimental Evidence from Energy Saving Programs

Identifying who should be treated is a central question in economics. There are two competing approaches to targeting - paternalistic and autonomous. In the paternalistic approach, policymakers optimally target the policy given observable individual characteristics. In contrast, the autonomous approach acknowledges that individuals may possess key unobservable information on heterogeneous policy impacts, and allows them to self-select into treatment. In this paper, we propose a new approach that mixes paternalistic assignment and autonomous choice. Our approach uses individual characteristics and empirical welfare maximization to identify who should be treated, untreated, and decide whether to be treated themselves. We apply this method to design a targeting policy for an energy saving programs using data collected in a randomized field experiment. We show that optimally mixing paternalistic assignments and autonomous choice significantly improves the social welfare gain of the policy. Exploiting random variation generated by the field experiment, we develop a method to estimate average treatment effects for each subgroup of individuals who would make the same autonomous treatment choice. Our estimates confirm that the estimated assignment policy optimally allocates individuals to be treated, untreated, or choose themselves based on the relative merits of paternalistic assignments and autonomous choice for individuals types.

==> mechanism_option_NvTvO_firststep_NvO.tex <==
\begin{tabular*}{.9\textwidth}{@{\extracolsep{\fill} } lccc }
\toprule
& \multicolumn{3}{c}{Optimal assignment} \\
& \multicolumn{3}{c}{in NT \& T \& O} \\
\cmidrule(l{3pt}r{3pt}){2-4}
& NT & T & O \\
Share & (19\%) & (37\%) & (44\%) \\
\midrule
\addlinespace
\textbf{A) Counterfactual analysis of opt-in policy}  &  &  \\
\addlinespace
Opt-in rate (if assigned to opt-in) & 41\% & 40\% & 37\%  \\
\addlinespace
LATE (Compilers of opt-in)  & -1600.9 & 187.7 & 1502.5\\
\addlinespace
LATE (Non-compilers of opt-in)  & -264.1 & 600.1 & -669.2\\
\midrule
\addlinespace
\textbf{B) Counterfactual analysis of each policy}  &  &  \\
\addlinespace
ITT (if assinged to NT) & \textcolor{red}{0} & 0 & 0\\
\addlinespace
ITT (if assinged to T)  & -806.3 & \textcolor{red}{437} & 130.5\\
\addlinespace
ITT (if assinged to O)  & -649.4 & 74.2 & \textcolor{red}{553.3} \\
\addlinespace
\bottomrule
\end{tabular*}


==> table/character_opt_COT_fs_CO_dep4to6.tex <==
\begin{table}[H]

\caption{\label{tab:unnamed-chunk-11}Characteristics of the three-option policies}
\centering
\begin{tabular}[t]{cccccccc}
\toprule
\multicolumn{6}{c}{ } & \multicolumn{2}{c}{LATE} \\
\cmidrule(l{3pt}r{3pt}){7-8}
Options & Depth & Recommend & OR & ITT-T & ITT-O & Complier & Non-Complier\\
\midrule
 &  & C & 0.36 & -303.31 & -559.30 & -1570.74 & 397.55\\

 &  & O & 0.40 & 76.64 & 558.56 & 1413.10 & -796.91\\

\multirow{-3}{*}{\centering\arraybackslash C, O \& T} & \multirow{-3}{*}{\centering\arraybackslash 4} & T & 0.36 & 235.06 & 126.62 & 353.62 & 168.94\\
\cmidrule{1-8}
 &  & C & 0.36 & -500.62 & -606.03 & -1663.24 & 165.83\\

 &  & O & 0.41 & 65.77 & 603.60 & 1466.66 & -913.97\\

\multirow{-3}{*}{\centering\arraybackslash C, O \& T} & \multirow{-3}{*}{\centering\arraybackslash 5} & T & 0.33 & 374.23 & 38.39 & 116.44 & 501.02\\
\cmidrule{1-8}
 &  & C & 0.38 & -592.82 & -579.48 & -1527.14 & -21.49\\

 &  & O & 0.40 & -0.17 & 668.63 & 1663.39 & -1118.34\\

\multirow{-3}{*}{\centering\arraybackslash C, O \& T} & \multirow{-3}{*}{\centering\arraybackslash 6} & T & 0.33 & 462.91 & -115.00 & -346.64 & 864.84\\
\bottomrule
\end{tabular}
\end{table}


==> table/character_opt_COT_fs_CT_dep4to6.tex <==
\begin{table}[H]

\caption{\label{tab:unnamed-chunk-4}Characteristics of the three-option policies}
\centering
\begin{tabular}[t]{cccccccc}
\toprule
\multicolumn{6}{c}{ } & \multicolumn{2}{c}{LATE} \\
\cmidrule(l{3pt}r{3pt}){7-8}
Options & Depth & Recommend & OR & ITT-T & ITT-O & Complier & Non-Complier\\
\midrule
 &  & C & 0.33 & -370.00 & -386.66 & -1164.79 & 24.93\\

 &  & O & 0.37 & 52.95 & 361.38 & 963.99 & -493.40\\

\multirow{-3}{*}{\centering\arraybackslash C, O \& T} & \multirow{-3}{*}{\centering\arraybackslash 4} & T & 0.40 & 387.37 & 139.54 & 352.73 & 410.04\\
\cmidrule{1-8}
 &  & C & 0.27 & -384.93 & -420.36 & -1535.82 & 48.79\\

 &  & O & 0.42 & -3.35 & 520.64 & 1245.35 & -900.45\\

\multirow{-3}{*}{\centering\arraybackslash C, O \& T} & \multirow{-3}{*}{\centering\arraybackslash 5} & T & 0.37 & 437.36 & -6.95 & -18.65 & 708.24\\
\cmidrule{1-8}
 &  & C & 0.26 & -372.96 & -303.97 & -1180.72 & -92.91\\

 &  & O & 0.48 & 56.48 & 553.58 & 1149.27 & -959.07\\

\multirow{-3}{*}{\centering\arraybackslash C, O \& T} & \multirow{-3}{*}{\centering\arraybackslash 6} & T & 0.29 & 429.46 & -140.81 & -482.77 & 805.10\\
\bottomrule
\end{tabular}
\end{table}


==> table/character_opt_COT_fs_OT_dep4to6.tex <==
\begin{table}[H]

\caption{\label{tab:unnamed-chunk-18}Characteristics of the three-option policies}
\centering
\begin{tabular}[t]{cccccccc}
\toprule
\multicolumn{6}{c}{ } & \multicolumn{2}{c}{LATE} \\
\cmidrule(l{3pt}r{3pt}){7-8}
Options & Depth & Recommend & OR & ITT-T & ITT-O & Complier & Non-Complier\\
\midrule
 &  & C & 0.39 & -59.11 & -286.10 & -728.25 & 373.85\\

 &  & O & 0.39 & 28.19 & 590.34 & 1529.99 & -915.33\\

\multirow{-3}{*}{\centering\arraybackslash C, O \& T} & \multirow{-3}{*}{\centering\arraybackslash 4} & T & 0.34 & 154.99 & -192.18 & -558.70 & 529.21\\
\cmidrule{1-8}
 &  & C & 0.35 & -384.93 & -316.16 & -915.84 & -105.03\\

 &  & O & 0.39 & 165.00 & 750.40 & 1941.39 & -954.23\\

\multirow{-3}{*}{\centering\arraybackslash C, O \& T} & \multirow{-3}{*}{\centering\arraybackslash 5} & T & 0.38 & 423.74 & -126.92 & -331.72 & 891.94\\
\cmidrule{1-8}
 &  & C & 0.32 & -518.53 & -463.38 & -1456.46 & -80.89\\

 &  & O & 0.40 & 222.10 & 835.62 & 2074.74 & -1027.25\\

\multirow{-3}{*}{\centering\arraybackslash C, O \& T} & \multirow{-3}{*}{\centering\arraybackslash 6} & T & 0.41 & 654.09 & 46.98 & 115.97 & 1020.56\\
\bottomrule
\end{tabular}
\end{table}


==> table/summary_camp2groups.tex <==
\begin{tabular*}{\textwidth}{@{\extracolsep{\fill} } lcc }
\toprule
&   Baseline group & Incentivized group \\ 
\midrule 
 Household income (JPY10,000) & 768.18  & 755.97 \\
 &  (343.46)  & (334.23) \\ \addlinespace
 Square Meters &  111.44  & 107.51 \\
 &  (31.09)  & (30.64) \\ \addlinespace
 Number of Bedrooms   & 3.84  & 3.76 \\
 & (1.15)  & (1.09) \\ \addlinespace
 Age of Building   & 15.59  & 15.14 \\
   & (11.68)  & (11.39) \\ \addlinespace
 Number of room AC   & 3.17  & 3.10 \\
  & (1.33)  & (1.34) \\ \addlinespace
 Number of TV   & 2.12  & 2.07 \\
   & (1.05)  & (1.10) \\ \addlinespace
 Number of refrigerator   & 1.13  & 1.12 \\
   & (0.38)  & (0.37) \\ \addlinespace
 Electricity usage (kWh/day)  in the pre-experimental period  & 13.09  & 13.02 \\
  & (5.58)  & (5.71) \\ \addlinespace
 
\specialrule{.1em}{.05em}{.05em} \end{tabular*}

==> table/testtable.tex <==
\begin{tabular*}{.9\textwidth}{@{\extracolsep{\fill} } cccccccc }
\toprule
\multicolumn{1}{c}{ } & \multicolumn{3}{c}{Optimal share} & & \multicolumn{3}{l}{Welfare gain relative to other policies}   \\
\cmidrule(l{3pt}r{3pt}){2-4} \cmidrule(l{3pt}r{3pt}){6-8}
Option &  C & O & T & & Compared to & $\Delta W^{ITT}$ & 95\% CI \\
\cmidrule(l{3pt}r{3pt}){1-4} \cmidrule(l{3pt}r{3pt}){6-8}
 &  &  &  & & 100\% C & 281.0 & (119.0,  443.0) \\
 C \& O & 29\% & 71\% & 0\% & & 100\% T & 222.2 & (42.6, 401.9) \\
 &  &  &  & & 100\% O & 138.6 & (36.9,  240.2) \\
\bottomrule
\end{tabular*}

==> table/testtable2.tex <==
\begin{tabular*}{.9\textwidth}{@{\extracolsep{\fill} } lcccc }
\toprule
 & \multicolumn{2}{c}{Peak hour usage} & \multicolumn{2}{c}{Peak hour usage}       \\
\multicolumn{1}{c}{ } & \multicolumn{2}{c}{$-$ Pre-peak hour usage} & \multicolumn{2}{c}{$-$ Post-peak hour usage}      \\ 
\cmidrule(l{3pt}r{3pt}){2-3} 
\cmidrule(l{3pt}r{3pt}){4-5} 
& Low & High & Low & High  \\ 
\midrule
100\% Treatment & -0.108  & -0.079  & -0.089  & -0.094  \\
      & (0.028) & (0.031) & (0.030) & (0.028) \\
      \addlinespace 
100\% Opt-in & -0.022  & -0.073  & -0.070  & -0.023  \\
      & (0.034) & (0.041) & (0.037) & (0.037) \\
      \midrule
      p-value (T = O) & 0.013  & 0.880  & 0.595  & 0.047  \\
      Opt-in rate & 36.92  & 37.44  & 39.85  & 34.69  \\
\bottomrule
\end{tabular*}

==> table/testtable3.tex <==

\begin{tabular*}{.9\textwidth}{@{\extracolsep{\fill} } lcccc }
\toprule
 & \multicolumn{2}{c}{Number of people at home} & \multicolumn{2}{c}{Interested in}       \\
\multicolumn{1}{c}{ } & \multicolumn{2}{c}{in peak hours} & \multicolumn{2}{c}{energy conservation}      \\ 
\cmidrule(l{3pt}r{3pt}){2-3} 
\cmidrule(l{3pt}r{3pt}){4-5} 
& Low & High & Low & High  \\ 
\midrule
100\% Treatment & -0.096  & -0.098  & -0.134  & -0.057  \\
        & (0.027) & (0.034) & (0.028) & (0.031) \\
        \addlinespace 
100\% Opt-in & -0.022  & -0.094  & -0.036  & -0.072  \\
        & (0.034) & (0.042) & (0.035) & (0.040) \\
        \midrule
        p-value (T = O) & 0.020  & 0.934  & 0.004  & 0.715  \\
        Opt-in rate & 37.64  & 36.57  & 33.83  & 40.55  \\
\bottomrule
\end{tabular*}



==> table/testtable4.tex <==

\begin{tabular*}{.5\textwidth}{@{\extracolsep{\fill} } lc }
\toprule
& (1) \\
\midrule
100\% Treatment & -0.097  \\
        & (0.021) \\
        \addlinespace 
100\% Opt-in & -0.052  \\
        & (0.027) \\
        \midrule
Observations & 1,176,480 \\
p-value (T = O) & 0.088  \\
Opt-in rate & 37.17  \\   
\bottomrule
\end{tabular*}



==> table/testtable5.tex <==

\begin{tabular*}{.9\textwidth}{@{\extracolsep{\fill} } lccc }
\toprule
 & \multicolumn{3}{c}{Optimal assignment}     \\
 & \multicolumn{3}{c}{in O \& T \& C policy}     \\
\cmidrule(l{3pt}r{3pt}){2-4} 
& O & T & C \\

Share & (36\%)  & (26\%) & (37\%) \\
\midrule
\addlinespace
\textbf{A) Counterfactual analysis of opt-in policy}  &  &  \\
\addlinespace
Opt-in rate (if assigned to opt-in) & 40\%  & 41\% & 32\% \\
\addlinespace
LATE (Compilers of opt-in)  &  2074.7 & 116.0 & -1456.5 \\
\addlinespace
LATE (Non-compilers of opt-in)  & -1027.3 & 1020.6 & -80.9  \\
\bottomrule
\end{tabular*}



==> table/testtable6.tex <==

\begin{tabular*}{.9\textwidth}{@{\extracolsep{\fill} } lccc }
\toprule
 & \multicolumn{3}{c}{Optimal assignment}     \\
 & \multicolumn{3}{c}{in O \& T \& C policy}     \\
\cmidrule(l{3pt}r{3pt}){2-4} 
& O & T & C \\

Share & (36\%)  & (26\%) & (37\%) \\
\midrule
\addlinespace
\textbf{A) Counterfactual analysis of opt-in policy}  &  &  \\
\addlinespace
Opt-in rate (if assigned to opt-in) & 40\%  & 41\% & 32\% \\
\addlinespace
LATE (Compilers of opt-in)  &  2074.7 & 116.0 & -1456.5 \\
\addlinespace
LATE (Non-compilers of opt-in)  & -1027.3 & 1020.6 & -80.9  \\
\midrule
\addlinespace
\textbf{B) Counterfactual analysis of each policy}  &  &  \\
\addlinespace
ITT (if assinged to O) & \textcolor{red}{835.6}  & 47.0  & -463.4  \\
\addlinespace
ITT (if assinged to T)  & 222.1 & \textcolor{red}{654.1} & -518.5 \\
\addlinespace
ITT (if assinged to C)  & 0  & 0 & \textcolor{red}{0} \\
\addlinespace
\bottomrule
\end{tabular*}



==> table/testtable7.tex <==
\begin{tabular*}{.9\textwidth}{@{\extracolsep{\fill} } lccc }
\toprule
 &  & \multicolumn{2}{c}{Peak hour usage}       \\
& & \multicolumn{2}{c}{$-$ Pre-peak hour usage}      \\ & & \multicolumn{2}{c}{(in pre-experiment)}      \\ 
\cmidrule(l{3pt}r{3pt}){3-4} 
& All &  Low & High  \\ 
\midrule
100\% Treatment & -0.097 & -0.108  & -0.079    \\
     & (0.021) & (0.028) & (0.031)  \\
      \addlinespace 
100\% Opt-in & -0.052 & -0.022  & -0.073    \\
     & (0.027) & (0.034) & (0.041)  \\
      \midrule
 Observations & 1,176,480  & 588,240 & 588,240 \\
 p-value (T = O) & 0.088 & 0.013  & 0.880    \\
      Opt-in rate & 37.17 & 36.92  & 37.44    \\
\bottomrule
\end{tabular*}


==> table/testtable_a1.tex <==
\scalebox{0.75}{
\begin{tabular*}{1.2\textwidth}{@{\extracolsep{\fill} } lccccccc }
\toprule
& C & T & O & C vs. T & C vs. O & T vs. O & ALL \\
\midrule
Peak hour usage (kWh)  & 0.192 & 0.19 & 0.189 & 0.609 & 0.633 & 0.961 & 0.838 \\
        & (0.004) & (0.004) & (0.005) &  &  &  &  \\
        \addlinespace 
Pre-peak hour usage (kWh) & 0.179 & 0.176 & 0.18 & 0.442 & 0.854 & 0.417 & 0.646 \\
        & (0.003) & (0.004) & (0.005) &  &  &  &  \\
        \addlinespace 
Post-peak hour usage (kWh)  & 0.299 & 0.297 & 0.293 & 0.756 & 0.426 & 0.588 & 0.725 \\
        & (0.004) & (0.004) & (0.006) &  &  &  &  \\
        \addlinespace 
Household income (JPY10,000) & 645.095 & 613.409 & 636.641 & 0.022 & 0.622 & 0.154 & 0.066 \\
        & (10.056) & (9.384) & (13.778) &  &  &  &  \\
        \addlinespace 
Number of people at home & 2.481 & 2.444 & 2.47 & 0.406 & 0.846 & 0.626 & 0.703 \\
        & (0.031) & (0.032) & (0.045) &  &  &  &  \\
        \addlinespace 
Interested in energy conservation & 3.45 & 3.464 & 3.488 & 0.647 & 0.299 & 0.517 & 0.584 \\
        & (0.022) & (0.022) & (0.029) &  &  &  &  \\
\bottomrule
\end{tabular*}
}

==> table/welfare_optCOT_depth6_v2.tex <==
\begin{tabular*}{.9\textwidth}{@{\extracolsep{\fill} } cccccccc }
\toprule
\multicolumn{1}{c}{ } & \multicolumn{3}{c}{Optimal share} & & \multicolumn{3}{l}{Welfare gain relative to other policies} \\
\cmidrule(l{3pt}r{3pt}){2-4} \cmidrule(l{3pt}r{3pt}){6-8}
Option & O & T & C & & Compared to & $\Delta W^{ITT}$ & 95\% CI \\
\cmidrule(l{3pt}r{3pt}){1-4} \cmidrule(l{3pt}r{3pt}){6-8}
\multirow{4}{*}{O \& T \& C} & \multirow{4}{*}{36\%} & \multirow{4}{*}{26\%} & \multirow{4}{*}{37\%} & & 100\% C & 475.4 & (327.9, 622.9) \\
 &  &  &  & & 100\% T & 416.6 & (261.2, 572.0) \\
 &  &  &  & & 100\% O & 333.0 & (185.0, 480.9) \\
 &  &  &  & & T \& C & 291.3 & (150.7, 431.8) \\
\bottomrule
\end{tabular*}


==> table/welfare_optCO_dep3_v2.tex <==
\begin{tabular*}{.9\textwidth}{@{\extracolsep{\fill} } cccccccc }
\toprule
\multicolumn{1}{c}{ } & \multicolumn{3}{c}{Optimal share} & & \multicolumn{3}{l}{Welfare gain relative to other policies} \\
\cmidrule(l{3pt}r{3pt}){2-4} \cmidrule(l{3pt}r{3pt}){6-8}
Option & C & O & T & & Compared to & $\Delta W^{ITT}$ & 95\% CI \\
\cmidrule(l{3pt}r{3pt}){1-4} \cmidrule(l{3pt}r{3pt}){6-8}
 &  &  &  & & 100\% C & 281.0 & (119.0, 443.0) \\
 C \& O & 29\% & 71\% & 0\% & & 100\% T & 222.2 & (42.6, 401.9) \\
 &  &  &  & & 100\% O & 138.6 & (36.9, 240.2) \\
\bottomrule
\end{tabular*}


==> table/welfare_optCT_dep3_v2.tex <==
\begin{tabular*}{.9\textwidth}{@{\extracolsep{\fill} } cccccccc }
\toprule
\multicolumn{1}{c}{ } & \multicolumn{3}{c}{Optimal share} & & \multicolumn{3}{l}{Welfare gain relative to other policies} \\
\cmidrule(l{3pt}r{3pt}){2-4} \cmidrule(l{3pt}r{3pt}){6-8}
Option & O & T & C & & Compared to & $\Delta W^{ITT}$ & 95\% CI \\
\cmidrule(l{3pt}r{3pt}){1-4} \cmidrule(l{3pt}r{3pt}){6-8}
 &  &  &  & & 100\% C & 184.2 & (57.8, 310.6) \\
 T \& C & 0\% & 52\% & 48\% & & 100\% T & 125.4 & (7.6, 243.1) \\
 &  &  &  & & 100\% O & 41.7 & (-146.1, 229.5) \\
\bottomrule
\end{tabular*}


==> table/welfare_optOT_dep3_v2.tex <==
\begin{tabular*}{.9\textwidth}{@{\extracolsep{\fill} } cccccccc }
\toprule
\multicolumn{1}{c}{ } & \multicolumn{3}{c}{Optimal share} & & \multicolumn{3}{l}{Welfare gain relative to other policies} \\
\cmidrule(l{3pt}r{3pt}){2-4} \cmidrule(l{3pt}r{3pt}){6-8}
Option & C & O & T & & Compared to & $\Delta W^{ITT}$ & 95\% CI \\
\cmidrule(l{3pt}r{3pt}){1-4} \cmidrule(l{3pt}r{3pt}){6-8}
 &  &  &  & & 100\% C & 346.0 & (164.1, 527.8) \\
 T \& O & 0\% & 52\% & 48\% & & 100\% T & 287.2 & (146.1, 428.2) \\
 &  &  &  & & 100\% O & 203.5 & (80.4, 326.6) \\
\bottomrule
\end{tabular*}


==> table/welfare_optOT_dep3_v2_noheader.tex <==
\begin{tabular*}{.9\textwidth}{@{\extracolsep{\fill} } cccccccc }
\toprule
\multicolumn{1}{c}{ } & \multicolumn{3}{c}{Optimal share} & & \multicolumn{3}{l}{Welfare gain relative to other policies} \\
\cmidrule(l{3pt}r{3pt}){2-4} \cmidrule(l{3pt}r{3pt}){6-8}
Option & C & O & T & & Compared to & $\Delta W^{ITT}$ & 95\% CI \\
\cmidrule(l{3pt}r{3pt}){1-4} \cmidrule(l{3pt}r{3pt}){6-8}
 &  &  &  & & 100\% C & 281.0 & (119.0, 443.0) \\
 C \& O & 29\% & 71\% & 0\% & & 100\% T & 222.2 & (42.6, 401.9) \\
 &  &  &  & & 100\% O & 138.6 & (36.9, 240.2) \\
\cmidrule(l{3pt}r{3pt}){1-4} \cmidrule(l{3pt}r{3pt}){6-8}
 &  &  &  & & 100\% C & 346.0 & (164.1, 527.8) \\
 T \& O & 0\% & 52\% & 48\% & & 100\% T & 287.2 & (146.1, 428.2) \\
 &  &  &  & & 100\% O & 203.5 & (80.4, 326.6) \\
\bottomrule
\end{tabular*}







==> table/welfare_opt_COT_fs_CO_dep4to6.tex <==
\begin{table}[H]

\caption{\label{tab:unnamed-chunk-10}Welfare performance of the three-option policies}
\centering
\begin{tabular}[t]{ccccccccc}
\toprule
\multicolumn{2}{c}{ } & \multicolumn{3}{c}{Share} & \multicolumn{2}{c}{ } & \multicolumn{2}{c}{95\% CI} \\
\cmidrule(l{3pt}r{3pt}){3-5} \cmidrule(l{3pt}r{3pt}){8-9}
Options & Depth & C & O & T & Benchmark & Welfare gain & Lower & Upper\\
\midrule
 &  &  &  &  & Unif. C & 307.06 & 146.54 & 467.57\\

 &  &  &  &  & Unif. O & 164.59 & 13.04 & 316.13\\

 &  &  &  &  & Unif. T & 248.25 & 115.12 & 381.37\\

\multirow{-4}{*}{\centering\arraybackslash C, O \& T} & \multirow{-4}{*}{\centering\arraybackslash 4} & \multirow{-4}{*}{\centering\arraybackslash 0.22} & \multirow{-4}{*}{\centering\arraybackslash 0.38} & \multirow{-4}{*}{\centering\arraybackslash 0.40} & C \& O, Depth 3 & 26.03 & -94.56 & 146.61\\
\cmidrule{1-9}
 &  &  &  &  & Unif. C & 392.70 & 230.58 & 554.83\\

 &  &  &  &  & Unif. O & 250.23 & 107.03 & 393.44\\

 &  &  &  &  & Unif. T & 333.89 & 191.99 & 475.80\\

\multirow{-4}{*}{\centering\arraybackslash C, O \& T} & \multirow{-4}{*}{\centering\arraybackslash 5} & \multirow{-4}{*}{\centering\arraybackslash 0.21} & \multirow{-4}{*}{\centering\arraybackslash 0.42} & \multirow{-4}{*}{\centering\arraybackslash 0.36} & C \& O, Depth 3 & 111.67 & 1.83 & 221.51\\
\cmidrule{1-9}
 &  &  &  &  & Unif. C & 465.92 & 301.82 & 630.02\\

 &  &  &  &  & Unif. O & 323.45 & 185.08 & 461.82\\

 &  &  &  &  & Unif. T & 407.11 & 262.19 & 552.02\\

\multirow{-4}{*}{\centering\arraybackslash C, O \& T} & \multirow{-4}{*}{\centering\arraybackslash 6} & \multirow{-4}{*}{\centering\arraybackslash 0.19} & \multirow{-4}{*}{\centering\arraybackslash 0.44} & \multirow{-4}{*}{\centering\arraybackslash 0.37} & C \& O, Depth 3 & 184.89 & 79.41 & 290.37\\
\bottomrule
\end{tabular}
\end{table}


==> table/welfare_opt_COT_fs_CT_dep4to6.tex <==
\begin{table}[H]

\caption{\label{tab:unnamed-chunk-3}Welfare performance of the three-option policies}
\centering
\begin{tabular}[t]{ccccccccc}
\toprule
\multicolumn{2}{c}{ } & \multicolumn{3}{c}{Share} & \multicolumn{2}{c}{ } & \multicolumn{2}{c}{95\% CI} \\
\cmidrule(l{3pt}r{3pt}){3-5} \cmidrule(l{3pt}r{3pt}){8-9}
Options & Depth & C & O & T & Benchmark & Welfare gain & Lower & Upper\\
\midrule
 &  &  &  &  & Unif. C & 293.16 & 128.65 & 457.67\\

 &  &  &  &  & Unif. O & 150.69 & 20.38 & 281.01\\

 &  &  &  &  & Unif. T & 234.35 & 79.65 & 389.06\\

\multirow{-4}{*}{\centering\arraybackslash C, O \& T} & \multirow{-4}{*}{\centering\arraybackslash 4} & \multirow{-4}{*}{\centering\arraybackslash 0.21} & \multirow{-4}{*}{\centering\arraybackslash 0.51} & \multirow{-4}{*}{\centering\arraybackslash 0.28} & C \& T, Depth 3 & 108.99 & -26.12 & 244.10\\
\cmidrule{1-9}
 &  &  &  &  & Unif. C & 380.09 & 215.59 & 544.58\\

 &  &  &  &  & Unif. O & 237.62 & 101.08 & 374.15\\

 &  &  &  &  & Unif. T & 321.28 & 168.43 & 474.12\\

\multirow{-4}{*}{\centering\arraybackslash C, O \& T} & \multirow{-4}{*}{\centering\arraybackslash 5} & \multirow{-4}{*}{\centering\arraybackslash 0.22} & \multirow{-4}{*}{\centering\arraybackslash 0.45} & \multirow{-4}{*}{\centering\arraybackslash 0.33} & C \& T, Depth 3 & 195.92 & 67.33 & 324.50\\
\cmidrule{1-9}
 &  &  &  &  & Unif. C & 381.83 & 219.25 & 544.42\\

 &  &  &  &  & Unif. O & 239.36 & 106.64 & 372.08\\

 &  &  &  &  & Unif. T & 323.02 & 162.61 & 483.44\\

\multirow{-4}{*}{\centering\arraybackslash C, O \& T} & \multirow{-4}{*}{\centering\arraybackslash 6} & \multirow{-4}{*}{\centering\arraybackslash 0.25} & \multirow{-4}{*}{\centering\arraybackslash 0.47} & \multirow{-4}{*}{\centering\arraybackslash 0.29} & C \& T, Depth 3 & 197.66 & 65.15 & 330.17\\
\bottomrule
\end{tabular}
\end{table}


==> table/welfare_opt_COT_fs_OT_dep4to6.tex <==
\begin{table}[H]

\caption{\label{tab:unnamed-chunk-17}Welfare performance of the three-option policies}
\centering
\begin{tabular}[t]{ccccccccc}
\toprule
\multicolumn{2}{c}{ } & \multicolumn{3}{c}{Share} & \multicolumn{2}{c}{ } & \multicolumn{2}{c}{95\% CI} \\
\cmidrule(l{3pt}r{3pt}){3-5} \cmidrule(l{3pt}r{3pt}){8-9}
Options & Depth & C & O & T & Benchmark & Welfare gain & Lower & Upper\\
\midrule
 &  &  &  &  & Unif. C & 322.37 & 155.95 & 488.80\\

 &  &  &  &  & Unif. O & 179.91 & 43.79 & 316.02\\

 &  &  &  &  & Unif. T & 263.56 & 114.99 & 412.14\\

\multirow{-4}{*}{\centering\arraybackslash C, O \& T} & \multirow{-4}{*}{\centering\arraybackslash 4} & \multirow{-4}{*}{\centering\arraybackslash 0.18} & \multirow{-4}{*}{\centering\arraybackslash 0.45} & \multirow{-4}{*}{\centering\arraybackslash 0.37} & O \& T, Depth 3 & -23.59 & -97.05 & 49.88\\
\cmidrule{1-9}
 &  &  &  &  & Unif. C & 407.38 & 255.61 & 559.15\\

 &  &  &  &  & Unif. O & 264.91 & 119.33 & 410.49\\

 &  &  &  &  & Unif. T & 348.57 & 197.70 & 499.44\\

\multirow{-4}{*}{\centering\arraybackslash C, O \& T} & \multirow{-4}{*}{\centering\arraybackslash 5} & \multirow{-4}{*}{\centering\arraybackslash 0.33} & \multirow{-4}{*}{\centering\arraybackslash 0.38} & \multirow{-4}{*}{\centering\arraybackslash 0.29} & O \& T, Depth 3 & 61.42 & -38.56 & 161.40\\
\cmidrule{1-9}
 &  &  &  &  & Unif. C & 475.43 & 327.91 & 622.95\\

 &  &  &  &  & Unif. O & 332.96 & 185.01 & 480.91\\

 &  &  &  &  & Unif. T & 416.62 & 261.19 & 572.05\\

\multirow{-4}{*}{\centering\arraybackslash C, O \& T} & \multirow{-4}{*}{\centering\arraybackslash 6} & \multirow{-4}{*}{\centering\arraybackslash 0.37} & \multirow{-4}{*}{\centering\arraybackslash 0.36} & \multirow{-4}{*}{\centering\arraybackslash 0.26} & O \& T, Depth 3 & 129.47 & 23.65 & 235.28\\
\bottomrule
\end{tabular}
\end{table}


==> table/welfare_opt_CO_dep3.tex <==
\begin{table}[H]

\caption{\label{tab:unnamed-chunk-9}Welfare performance of the two-option policy}
\centering
\begin{tabular}[t]{ccccccccc}
\toprule
\multicolumn{2}{c}{ } & \multicolumn{3}{c}{Share} & \multicolumn{2}{c}{ } & \multicolumn{2}{c}{95\% CI} \\
\cmidrule(l{3pt}r{3pt}){3-5} \cmidrule(l{3pt}r{3pt}){8-9}
Options & Depth & C & O & T & Benchmark & Welfare gain & Lower & Upper\\
\midrule
 &  &  &  &  & Unif. C & 281.03 & 119.03 & 443.03\\

 &  &  &  &  & Unif. O & 138.56 & 36.93 & 240.19\\

\multirow{-3}{*}{\centering\arraybackslash C \& O} & \multirow{-3}{*}{\centering\arraybackslash 3} & \multirow{-3}{*}{\centering\arraybackslash 0.29} & \multirow{-3}{*}{\centering\arraybackslash 0.71} & \multirow{-3}{*}{\centering\arraybackslash 0} & Unif. T & 222.22 & 42.57 & 401.87\\
\bottomrule
\end{tabular}
\end{table}


==> table/welfare_opt_CT_dep3.tex <==
\begin{table}[H]

\caption{\label{tab:unnamed-chunk-2}Welfare performance of the two-option policy}
\centering
\begin{tabular}[t]{ccccccccc}
\toprule
\multicolumn{2}{c}{ } & \multicolumn{3}{c}{Share} & \multicolumn{2}{c}{ } & \multicolumn{2}{c}{95\% CI} \\
\cmidrule(l{3pt}r{3pt}){3-5} \cmidrule(l{3pt}r{3pt}){8-9}
Options & Depth & C & O & T & Benchmark & Welfare gain & Lower & Upper\\
\midrule
 &  &  &  &  & Unif. C & 184.17 & 57.75 & 310.59\\

 &  &  &  &  & Unif. O & 41.70 & -146.09 & 229.50\\

\multirow{-3}{*}{\centering\arraybackslash C \& T} & \multirow{-3}{*}{\centering\arraybackslash 3} & \multirow{-3}{*}{\centering\arraybackslash 0.48} & \multirow{-3}{*}{\centering\arraybackslash 0} & \multirow{-3}{*}{\centering\arraybackslash 0.52} & Unif. T & 125.36 & 7.58 & 243.15\\
\bottomrule
\end{tabular}
\end{table}


==> table/welfare_opt_OT_dep3.tex <==
\begin{table}[H]

\caption{\label{tab:unnamed-chunk-16}Welfare performance of the two-option policy}
\centering
\begin{tabular}[t]{ccccccccc}
\toprule
\multicolumn{2}{c}{ } & \multicolumn{3}{c}{Share} & \multicolumn{2}{c}{ } & \multicolumn{2}{c}{95\% CI} \\
\cmidrule(l{3pt}r{3pt}){3-5} \cmidrule(l{3pt}r{3pt}){8-9}
Options & Depth & C & O & T & Benchmark & Welfare gain & Lower & Upper\\
\midrule
 &  &  &  &  & Unif. C & 345.96 & 164.08 & 527.84\\

 &  &  &  &  & Unif. O & 203.49 & 80.43 & 326.55\\

\multirow{-3}{*}{\centering\arraybackslash O \& T} & \multirow{-3}{*}{\centering\arraybackslash 3} & \multirow{-3}{*}{\centering\arraybackslash 0} & \multirow{-3}{*}{\centering\arraybackslash 0.52} & \multirow{-3}{*}{\centering\arraybackslash 0.48} & Unif. T & 287.15 & 146.06 & 428.24\\
\bottomrule
\end{tabular}
\end{table}


==> welfare_option_NvT.tex <==
\begin{tabular*}{.9\textwidth}{@{\extracolsep{\fill} } cccccccc }
\toprule
\multicolumn{1}{c}{ } & \multicolumn{3}{c}{Optimal share} & & \multicolumn{3}{l}{Welfare gain relative to other policies} \\
\cmidrule(l{3pt}r{3pt}){2-4} \cmidrule(l{3pt}r{3pt}){6-8}
Option & NT & T & O & & Compared to & $\Delta W^{ITT}$ & 95\% CI \\
\cmidrule(l{3pt}r{3pt}){1-4} \cmidrule(l{3pt}r{3pt}){6-8}
 &  &  &  & & 100\% NT & 219.0 & (89.7, 348.3) \\
NT \& T & 48\% & 52\% & 0\% & & 100\% T & 152.6 & (36.6, 268.6) \\
 &  &  &  & & 100\% O & 70.6 & (-118.1, 259.4) \\
\bottomrule
\end{tabular*}


==> welfare_option_NvTvO_firststep_NvO.tex <==
\begin{tabular*}{.9\textwidth}{@{\extracolsep{\fill} } cccccccc }
\toprule
\multicolumn{1}{c}{ } & \multicolumn{3}{c}{Optimal share} & & \multicolumn{3}{l}{Welfare gain relative to other policies} \\
\cmidrule(l{3pt}r{3pt}){2-4} \cmidrule(l{3pt}r{3pt}){6-8}
Option & NT & T & O & & Compared to & $\Delta W^{ITT}$ & 95\% CI \\
\cmidrule(l{3pt}r{3pt}){1-4} \cmidrule(l{3pt}r{3pt}){6-8}
\multirow{4}{*}{NT \& T \& O} & \multirow{4}{*}{19\%} & \multirow{4}{*}{44\%} & \multirow{4}{*}{37\%} & & 100\% NT & 405.5 & (238.7, 572.4) \\
 &  &  &  & & 100\% T & 339.1 & (194.0, 484.2) \\
 &  &  &  & & 100\% O & 257.2 & (115.9, 398.5) \\
 &  &  &  & & NT \& T &186.5 & (42.8, 330.2) \\
\bottomrule
\end{tabular*}

